The Variable Hierarchy for the Games mu-Calculus

Parity games are combinatorial representations of closed Boolean mu-terms. By adding to them draw positions, they have been organized by Arnold and one of the authors into a mu-calculus. As done by Berwanger et al. for the propositional modal mu-calculus, it is possible to classify parity games into levels of a hierarchy according to the number of fixed-point variables. We ask whether this hierarchy collapses w.r.t. the standard interpretation of the games mu-calculus into the class of all complete lattices. We answer this question negatively by providing, for each n >= 1, a parity game Gn with these properties: it unravels to a mu-term built up with n fixed-point variables, it is semantically equivalent to no game with strictly less than n-2 fixed-point variables.

==> macros.tex <==
%% PACKAGES
\RequirePackage{comment}
\RequirePackage{ifthen}

\newcommand{\myqed}{}

%% WORKING VERSION
\def\workingversion{}
\ifthenelse{\isundefined{\workingversion}}%
{%
\excludecomment{workingversion}
\includecomment{cleanversion}
}
{
\includecomment{workingversion}
\excludecomment{cleanversion}
}

\newenvironment{longversion}{}{}
\begin{workingversion}
  \newenvironment{tbs}{%
    \renewcommand{\labelitemi}{$\blacktriangleright$}%
    \begin{itemize}\tt }{\end{itemize}}
  %%
  \newcommand{\shtbs}[1]{\begin{tbs} \item #1 \end{tbs}}
  %%
  \newcommand{\tobesaid}[1]{\shtbs{#1}}
  %%
\end{workingversion}

\begin{cleanversion}
  \newcommand{\tobesaid}[1]{}
\end{cleanversion}

%% SPACES
\newcommand{\myhspace}[1]{\mbox{\hspace{#1}}}

%% ENVIRONMENTS
%%\itemsep=0mm
% \newenvironment{myitemize}[1][$\bullet$]{%
%   \begin{list}{#1}{%
%       \leftmargin=2.2mm%
%       \labelsep=1mm%
%       \itemsep=0mm%
%       \labelwidth=1mm%
%       \parsep=1mm
% }%
% }{\end{list}}

\newenvironment{myitemize}[1][$\bullet$]
{\begin{itemize}}{\end{itemize}}

\newenvironment{myenumerate}{%
  \setcounter{enumi}{0}
  \begin{list}{\theenumi}{%
      \leftmargin=2.2mm%
      \labelsep=1mm%
      \itemsep=0mm%
      \labelwidth=1mm%
      \parsep=1mm
}%
}{\stepcounter{enumi}\end{list}}

%%
\newcommand{\mymod}{\,\mathrm{mod}\,}
\newcommand{\hier}[1]{\mathcal{L}(#1)}
\newcommand{\card}[1]{|#1|}
\newcommand{\Ent}[1]{{\cal E}(#1)}
\newcommand{\ET}[1]{\widetilde{{\cal E}}(#1)}
\newcommand{\ETT}[1]{\widehat{{\cal E}}(#1)}
\newcommand{\HT}[1]{\widehat{#1}}
\newcommand{\WT}[1]{\widetilde{#1}}
\newcommand{\BL}[1]{{#1}_{\bullet}}
\newcommand{\BBL}[1]{{#1}_{\bullet \bullet}}
\newcommand{\Type} {\mathbb{T}}
\newcommand{\Pip}{\Pi^{+}}

\newcommand{\rTo}{\longrightarrow}

\newcommand{\set}[1]{\{\,#1\,\}}
\newcommand{\couple}[1]{\{#1\}}

\newcommand{\id}{\mathtt{id}} 

\newcommand{\tiff}{\text{ iff }}
\newcommand{\tif}{\text{ if }}
\newcommand{\tand}{\text{ and }}
\newcommand{\timplies}{\text{ implies }}
\newcommand{\tor}{\text{ or }}
\newcommand{\tst}{\text{ s.t. }}
\newcommand{\twith}{\text{ with }}

\newlength{\myhidel}
\newcommand{\myhide}[1]{%
  \settowidth{\myhidel}{$#1$}%
  \mbox{\hspace{\myhidel}}%
}

\newcounter{casecounter}
\def\thecasecounter{(\roman{casecounter})}
\newenvironment{proofbycases}[1][0]{
  \setcounter{casecounter}{#1}%
}{}

\newenvironment{caseinproof}{%
  \refstepcounter{casecounter}%
  %\ifthenelse{\equal{casecounter}{1}}{}{\par}%
  \vskip 1pt
  \noindent%
  \emph{Case~\thecasecounter.}~
}{\par}

\newcommand{\acompleter}{\par\ldots A COMPLETER \ldots \par}
\newcommand{\acompleterdici}{\par\ldots A COMPLETER D'ICI\ldots \par}
\newcommand{\EXERCICEPOURWALID}{\par\ldots EXERCICE POUR WALID \ldots
  \par}

%% CORRECTIONS 

\newcommand{\acomment}[2]{$-\!\!\!\!>$ \emph{#1} $<\!\!\!\!-$\footnote{#2}}
\newcommand{\luigi}{\emph{Luigi suggestion}:~ }


%% SECTIONING
\newcommand{\breath}{\vskip 6pt}
\newcommand{\myparagraph}[1]{\breath\par\noindent\textbf{#1}~}



\renewcommand{\lefteqn}[2][0mm]{\makebox[#1][l]{$#2$}}


%\newcommand{\card}{\mathrm{card}\,}
%\newcommand{\dom}{\mathrm{dom}\,}
%\newcommand{\cod}{\mathrm{cod}\,}
\newcommand{\desc}[1]{\overline{#1}}
\newcommand{\eql}{\bigl [}
\newcommand{\eqr}{\bigr ]}
% \newcommand{\homl}{\bigl \langle}
% \newcommand{\homr}{\bigr \rangle}
\newcommand{\homl}{\langle}
\newcommand{\homr}{\rangle}
\newcommand{\Mod}[1]{\mathrm{#1}}
\newcommand{\Theory}[1]{\mathbb{#1}}
%\newcommand{\mod}{\,\mathrm{mod}\,}
\renewcommand{\cong}{\equiv}
\newcommand{\reach}[1]{\overline{#1}}
\newcommand{\chain}{\sqsubset}
\newcommand{\schain}{\sqsubset_{\sigma}}
\newcommand{\pchain}{\sqsubset_{\pi}}
\newcommand{\comps}{||}
\newcommand{\compp}{\star}
\newcommand{\hide}{\backslash}
\newcommand{\TBE}{\mathcal{L}}
\newcommand{\Jprim}{\mathcal{K}}
\newcommand{\nnumbers}{\mathbb{N}}

%\newcommand{\Rho}{\Re}
\newcommand{\Rho}{\Upsilon}

\newcommand{\simulates}[1][]{\vartriangleright_{#1}}
\newcommand{\source}{\delta_{0}}
\newcommand{\target}{\delta_{1}}

%\renewcommand{\above}{\rightarrow^{*}}
\renewcommand{\above}{\text{ is an ancestor of }}
%\newcommand{\below}{\text{ is in the subtree of }}


%%%%%%%%%%%%%%%%%
%%% xypic
%%%%%%%%%%%%%%%%%


\newcommand{\myxygraph}[2][6em]{
  \mbox{$\begin{array}{@{\hspace{0mm}}c@{\hspace{0mm}}}
      \xy\xygraph{!{<#1,0cm>:<0cm,#1>::}#2}\endxy
    \end{array}$}
  }

%\def\deplacement{d(0.1)r(0.2)}
%\newgraphescape{p}[1]{[]*+{#1}([u(0.5)r(0.2)]*+{\pi})}

%\newgraphescape{p}[1]{[]*+{#1}*\cir{}="P"([d(0.2)r(0.4)]*+{\pi})}
\newgraphescape{p}[1]{[]*+{#1}*\cir{}="P"([d(0.2)r(0.4)]*+{\textrm{A}})}
%\newgraphescape{P}[1]{[]*++{#1}*\cir{}="P"([d(0.12)r(0.29)]*+{\pi})}
\newgraphescape{P}[1]{[]*++{#1}*\cir{}="P"([d(0.12)r(0.29)]*+{A})}
%\newgraphescape{s}[1]{[]*+{#1}*\cir{}="P"([d(0.2)r(0.4)]*+{\sigma})}
\newgraphescape{s}[1]{[]*+{#1}*\cir{}="P"([d(0.2)r(0.4)]*+{\textrm{E}})}
\newgraphescape{o}[1]{[]*+{#1}*\cir{}}
\newgraphescape{O}[1]{[]*++{#1}*\cir{}}

\newgraphescape{g}[1]{%
  []!s{v_{#1,1}}(:[l]!o{x_{#1,1}})
  :[d]!p{v_{#1,2}}(:[l]!o{x_{#1,2}})
  :[d]!s{v_{#1,3}}(:[l]!o{x_{#1,3}})
  :[d]!p{v_{#1,4}}(:[l]!o{x_{#1,4}})
  :[d]!s{v_{#1,5}}(:[l]!o{x_{#1,5}})
  "P"="E_{#1}"
}




\newgraphescape{a}[1]{[]*+{#1}*\frm{o}="P"([d(0.2)r(0.4)]*+{\pi})}
\newgraphescape{b}[1]{[]*+{#1}*\frm{o}="P"([d(0.2)r(0.4)]*+{\sigma})}
\newgraphescape{c}[1]{[]*+{#1}*\frm{o}}

\newgraphescape{j}[1]{%
  []!b{a_{#1,1}}(:[l]!c{x_{#1,1}})"P"="B_{#1}"
  :[d]!a{a_{#1,2}}(:[l]!c{x_{#1,2}})
  :[d]!b{a_{#1,3}}(:[l]!c{x_{#1,3}})
  :[d]!a{a_{#1,4}}(:[l]!c{x_{#1,4}})
  :[d]!b{a_{#1,5}}(:[l]!c{x_{#1,5}})
  "P"="E_{#1}"
}


%\newgraphescape{p}#1{[]*+[F]+[]{#1}} 
% \newgraphescape{p}#1{[]*=<1.6em>[o]{#1}*\frm{o}} 

% \newgraphescape{g}#1{
%   []="S"[d(0.05)]
%   ( -[d(0.6)d(0.6)l(0.6)]-[r(0.6)r(0.6)]-[r(0.6)l(0.6)],
%    -[d(0.6)d(0.6)r(0.6)]="RD")
%  [d(0.8)]*{#1}
% }

% \newgraphescape{G}#1{
%   []*{:}
%   [r(0.6)u(0.8)]
%   ( -[d(0.6)d(0.6)l(0.6)]-[r(0.6)r(0.6)]-[r(0.6)l(0.6)],
%    -[d(0.6)d(0.6)r(0.6)])
%  [d(0.8)]*{#1}
%  [r(0.6)]*{:}
% }


\newcommand\strategy[4][4]{
 \xy\xygraph{!{<#1pc,0pc>:<0pc,3pc>::} 
     []*{\firstplayer{#2}} [d]*{\secondplayer{#2}}
   #3
       }
   \endxy
 \hspace{10mm}
  \xy\xygraph{!{<#1pc,0pc>:<0pc,3pc>::} 
     #4
      }
  \endxy
  }

\newcommand\strategyw[4][4]{
 \xy\xygraph{!{<#1pc,0pc>:<0pc,3pc>::} 
     %[]*{\firstplayer{#2}} [d]*{\secondplayer{#2}}
   #3
       }
   \endxy
 \hspace{10mm}
  \xy\xygraph{!{<#1pc,0pc>:<0pc,3pc>::} 
     #4
      }
  \endxy
  }


% \newgraphescape{w}#1#2{
%   []!p{\firstplayer{#1}}="S" (:[r]!p{\firstvariable{#2}}) 
%   :[d]!p{\secondplayer{#1}} (:[r]!p{\secondvariable{#2}})
%   :[d]!p{\firstplayer{#1}} (:[r]!p{\thirdvariable{#2}}) 
%  }

% \newcommand{\firstvariable}[1]{\ifx#1a a_{0}\else b_{0}\fi}
% \newcommand{\secondvariable}[1]{\ifx#1a a_{1}\else b_{1}\fi}
% \newcommand{\thirdvariable}[1]{\ifx#1a a_{2}\else b_{2}\fi}
\newcommand{\firstvariable}[1]{\ifthenelse{\equal{#1}{a}}{a_{0}}{b_{0}}}
\newcommand{\secondvariable}[1]{\ifthenelse{\equal{#1}{a}}{a_{1}}{b_{1}}}
\newcommand{\thirdvariable}[1]{\ifthenelse{\equal{#1}{a}}{a_{2}}{b_{2}}}
\newcommand{\firstplayer}[1]{#1}
%\newcommand{\secondplayer}[1]{\ifx#1\pi\sigma \else \pi \fi}
\newcommand{\secondplayer}[1]{
  \ifthenelse{\equal{#1}{\pi}}{\sigma}{
    \ifthenelse{\equal{#1}{\sigma}}{\pi}{
      \ifthenelse{\equal{#1}{M}}{O}{M}
      }
    }
}

\ifx\TAC\undefined
\RequirePackage{ifthen}
\newcommand{\Whitstar}{}
\newcommand{\Whitvariablea}{a_{0}}
\newcommand{\Whitvariableb}{a_{1}}
\newcommand{\Whitvariablec}{a_{2}}
\newcommand{\Whitlabel}[3]{
  \ifthenelse{\equal{#2}{\pi}}{\renewcommand{\Whitstar}{}}
  {\renewcommand{\Whitstar}{*}}
  \ifthenelse{\equal{#3}{a}}{
   \renewcommand{\Whitvariablea}{a_{0}}
   \renewcommand{\Whitvariableb}{a_{1}}
   \renewcommand{\Whitvariablec}{a_{2}}
   }
  {\renewcommand{\Whitvariablea}{b_{0}}
   \renewcommand{\Whitvariableb}{b_{1}}
   \renewcommand{\Whitvariablec}{b_{2}}}
 W_{#1}^{\Whitstar}(\Whitvariablea,\Whitvariableb,\Whitvariablec)
}
\newgraphescape{A}#1#2#3#4#5{
  []!p{\firstplayer{#2}}="S"
  ( -[l(#4)]-[d(#5)]-[d(#5)]-[r(#4)]!p{\firstplayer{#2}}="B",
  -[r(#4)]-[d(#5)]-[d(#5)]-"B")
  [d(#5)]*{\Whitlabel{#1}{#2}{#3}}
  "B"
}
\newgraphescape{T}#1#2#3{[]!A{#1}{#2}{#3}{0.5}{0.8} }

% \newcommand{\mylabel}[1]{
%   \write\@auxout{\string
%     \newlabel{#1}{{\theenumi}{\thepage}}}
%     }
% \def\mylabel#1{\@bsphack\if@filesw {\let\thepage\relax
%    \xdef\@gtempa{\write\@auxout{\string
%       \newlabel{#1}{{\theenumi}{\thepage}}}}}\@gtempa
%    \if@nobreak \ifvmode\nobreak\fi\fi\fi\@esphack}
% \def\refcounter#1{\edef\@currentlabel{\csname p@#1\endcsname\csname the#1\endcsname}}
\fi


%%%%%%%%%%%%%%%%%%%%%%%
%%% Imported from FOSSACS03
\newcommand{\usubseteq}{\mathbin{\begin{rotate}{45}
        $\subseteq$\end{rotate}}}
\newcommand{\dsubseteq}{\mathbin{\begin{rotate}{-45}
        $\subseteq$\end{rotate}}}

\newcommand{\header}[1]{\par\noindent\textbf{#1}} %% header
\def\N{\mathbb{N}} %% natural numbers
%%def\set#1{\{#1\}} %% set former
%\newcommand{\rTo}{\longrightarrow} %% arrow to right.
\newcommand{\immprec}{\mapsto} %% out of component rel.
%\newcommand{\homl}{$\langle\!\langle$} %% left Mediator game delimiter
%\newcommand{\homr}{$\rangle\!\rangle$} %% right Mediator game delimiter
%\newcommand{\card}{\mathrm{card}\,} %% cardinality
\newcommand{\quotient}{\mbox{$/\hspace{-0.3em}\sim$}} %% quotient with \sim 
\newcommand{\Land}[1][]{{\textstyle\bigwedge_{#1}}} %% bigwedge
\newcommand{\Lor}[1][]{{\textstyle\bigvee_{\!\!#1\,}}} %% bogvee
\newcommand{\eval}[1]{|\!|#1|\!|} %% logical interpretation
\newcommand{\mscc}[1]{[\,#1\,]} %% maximal strongly connected component









%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "0"
%%% End: 


==> mylatex8.tex <==
\newcommand{\email}[1]{{\tt #1}}
\newcommand{\affiliation}[1]{#1}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "0"
%%% End: 

